Learning Dense UV Completion for Human Mesh Recovery

Human mesh reconstruction from a single image is challenging in the presence of occlusion, which can be caused by self, objects, or other humans. Existing methods either fail to separate human features accurately or lack proper supervision for feature completion. In this paper, we propose Dense Inpainting Human Mesh Recovery (DIMR), a two-stage method that leverages dense correspondence maps to handle occlusion. Our method utilizes a dense correspondence map to separate visible human features and completes human features on a structured UV map dense human with an attention-based feature completion module. We also design a feature inpainting training procedure that guides the network to learn from unoccluded features. We evaluate our method on several datasets and demonstrate its superior performance under heavily occluded scenarios compared to other methods. Extensive experiments show that our method obviously outperforms prior SOTA methods on heavily occluded images and achieves comparable results on the standard benchmarks (3DPW).

==> sections/3-methods.tex <==

\section{Method}
\label{chapter:method}
\subsection{Overview}

We propose DIMR to deal with the occlusions challenge in human reconstruction. Specifically, we focus on separating visible human instances and filling in missing information from context features (\emph{e.g.}, the background, and visible body parts) in a more effective way. 

% In our investigation, we observed that current top-down approaches rely heavily on bounding boxes to represent human instances, with the network trained to predict the human located at the center of the image while treating other humans as interruptions. However, we discovered that inaccurate bounding boxes generated from crowded scenes or heavily occluded humans can lead to network failure. Conversely, bottom-up approaches often use human-center heatmaps or feature vectors to represent different targets. Despite this, we found that most of these methods lack feature-level human separation design, making them insufficient in cases of incomplete bounding boxes or close human overlap.
% Given the limitations of the two methods, we developed DIMR to accurately extract visible features of the subject and infer invisible features during its design. 

We used dense correspondent maps and instance segmentations to model the human body, which provides a more accurate boundary than traditional top-down methods that use bounding boxes for human recognition and extraction. Through the dense map, we extract more accurate human body features. 
We also proposed an attention mechanism to selectively fuse features from the standardized dense map. Given the characteristics of the dense map, only 50 \% of its area can be effectively utilized each time, and feature fusion based on the dense map has a natural completion characteristic, even when the human body is completely unobstructed.


Lastly, we introduced a novel parallel training method, which trains the network in parallel with and without occlusion. And we directly supervise the occluded feature with the intact one. With direct feature supervision from, the network learned how to complete obstructed features from the visible parts, further improving its accuracy in separating human instances and filling in missing information from relevant features.

We rely on SMPL~\cite{smpl} parametric model to recover human mesh. SMPL represents a 3D mesh with $ \mathcal{M}(\boldsymbol{\theta}, \boldsymbol{\beta}) \in \mathbb{R}^{6890 \times 3}$ with \, $\boldsymbol{\theta} \in \mathbb{R}^{24 \times 3}$ , the first 10 coefficients for SMPL's PCA shape, and $\boldsymbol{\beta} \in \mathbb{R}^{10}$, the  joints rotations which include global rotations. We also use weak perspective camera model $\boldsymbol{\pi}=(s, t_x, t_y)$ to project the predicted body model to the image plane. 

Our model is generally a top-down method. Given an image, a detector will detect all the possible humans with bounding boxes. An input image $\mathbf{I} \in \mathbb{R}^{3 \times H \times W}$ is cropped by the bounding box and resized to a uniform shape, our regression model $D$ will directly regress parameters $(\boldsymbol{\theta}, \boldsymbol{\beta}, \boldsymbol{\pi})$ based on the image $\mathbf{I}$.


% DIMR was developed with the objective of addressing general occlusions and with the specific purpose of effectively separating visible human instances and filling in missing information from relevant features such as the background and visible human body parts. Currently, top-down approaches frequently utilize bounding boxes to represent human instances, with the network trained to predict the human located at the center of the image while other humans are treated as interruptions. However, inaccurate bounding boxes generated from crowded scenes or heavily occluded humans may result in network failure. Conversely, bottom-up approaches typically employ human center heatmaps or feature vectors to represent different targets. Nevertheless, due to variations in resolution and human scale, most of these methods lack feature-level human separation design. While they can address inter-human occlusion, the majority rely on losses to regulate human occlusions and are unable to differentiate between different human features. These methods prove insufficient in the case of an incomplete bounding box or close human overlap. Based on the limitations of the two methods mentioned above, DIMR considers both the accurate extraction of visible features of the subject and the inference of invisible features during its design. We utilize dense correspondent maps and instance segmentation to model the human body, which provides a more accurate boundary than traditional top-down methods that use bounding boxes for human recognition and extraction. With the dense map, we can extract more accurate human body features. Furthermore, we propose an attention mechanism to fuse features from the standardized dense map. Due to the characteristics of the dense map, only 50 \% of its area can be effectively utilized each time, therefore, feature fusion based on the dense map has a natural completion characteristic, even when the human body is completely unobstructed. Finally, we introduce a new parallel training method, which trains the network in parallel with and without occlusion. The network will further learn how to complete the obstructed features from the outside.\

\begin{figure*}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{pictures/pipeline.png}
  \hfill
  \vspace{-10pt}
  \caption{\textbf{\Ours pipeline overview}. Our pipeline consists of two network parts. (a) 6D pose calibration network take cropped human image as input and estimate human body translation and rotation. (b) The body pose network take cropped human image as input as well, and the estimated 6D pose will be concatenated be image features extracted by backbone as a condition to estimate a weak-perspective transformation $(s, t_{x}, t_{y})$ and body pose $\theta_{J}$ and shape $\beta$. The projection loss use perspective and weak-perspective re-projection loss simultaneously. The perspective projection use focal length $f=s \times z$ and supervise with key-points $J_{2D}^{ori}$ in original image coordinates before cropped.  The weak-perspective projection use $(s, t_{x}, t_{y})$, and use focal length of 5000 (pixels) and supervise with the  $J_{2D}^{im}$ in the cropped image coordinate.}
  \label{fig:pipeline}
\end{figure*}
\subsection{UV Based Feature Wrapping}
To better reasoning the occlusion, we propose to extract visible information via a dense corespondence $UV$ map. The $UV$ map is generated based on the SMPL model, every vertices as a set coordinate on this $UV$ map. Thus, the value of the $UV$ map could represents the state of a vertice. For a $UV$ position map, the 3 dimensional vaule represents the position of the vertice. And in our model, we wrap the image feature to $UV$ map, which means every feature vector on the map represents a feature for a particular part of the human. By predicting a $IUV$ map of the human body in an image, we are able to transfer the image feature to the $UV$ feature map with. We establish a dense pixel-mesh correspondence through this transfer. This correspondence provided DIMR with ordered human part features, which made it easier to recognize and utilize these image features.


Given the input image $I$, our mode will first predict the $IUV$ map $M_{iuv} \in \mathbb{R}^{3 \times H \times W}$, which the first channel $i\in \mathbb{R}^{H \times W}$ represents the segmentation of the human object, and the second and third channel are a two-dimensional coordinate $(u,v)\in \mathbb{R}^{2 \times H \times W}$, which represents the wrapped location of this pixel. 

$I$ is also passed through a image encoder to obtain an feature map $\mathbf{F_{img}} \in \mathbb{R}^{D \times H^{\prime} \times W^{\prime}}$. We choose HRNet \cite{cheng2020higherhrnet} as the image encoder. Compared to ResNet\cite{resnet}, HRNet's design preserves more image-aligned feautre and have a larger feature map output, which makes our wrapped feature more presice and correspond to the image pixel.

The predicted $IUV$ map is utilized to inverse wrap the feature vector on the feature map $\mathbf{F_{img}}$ into a $UV$ feature map $\mathbf{F_{UV} } \in \mathbb{R}^{D \times H^{\prime} \times W^{\prime}}$. Given the predicted $M_{iuv}$, we assign the feature vector to the $UV  \in \mathbb{R}^{D \times H^{\prime} \times W^{\prime}}$ map
 according to the following equations:
 \begin{equation}
 \centering
 \begin{split}
 \mathbf{F_{UV} }(u(x,y),v(x,y)) = F_{img}(x,y), i(x,y)>0\\
    x=0,1,...,(H^{\prime}-1), y=0,1,...,(W^{\prime}-1) 
\end{split}
\end{equation}

\textcolor{red}{ To avoid incorrect $UV$ wrapping, we utilize the $UV$ mask based on the ground-truth $UV$ map to filter out outlie features.} 



% We utilized an off-the-shelf Dense IUV detection method Densepose to predict the IUV map $M_{iuv}$ from the input large scale image.
\begin{figure}[t]
  \centering
%   \begin{subfigure}{0.45\textwidth}
%     \centering
%       \includegraphics[width=1\linewidth]{pictures/dollyzoom.pdf}
%       \caption{Solving distance ambiguity with distortion. This figure vividly demonstrates the dolly-zoom effect. We can fix the scale of the human by simultaneously adjusting focal length and the camera distance. The $Error$ indicates the NME error in the image space when using weak-perspective projection.
       
%     %   2D joint $L1$ error in pixel compared to weak-perspective projection under the same scale.
%       }
%       \label{fig:dollyzoom}
%   \end{subfigure}

    % \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{pictures/uv.png}
    \caption{IUV IUIUV VIUV IUV IUV IUV IUV IUV  IUV IUIUV VIUV IUV IUV IUV IUV IUV IUV IUIUV VIUV IUV IUV IUV IUV IUV IUV IUIUV VIUV IUV IUV IUV IUV IUV IUV IUIUV VIUV IUV IUV IUV IUV IUVn.}
    \label{fig:iuv_wrapping}
    % \end{subfigure}
    
% \caption{Solving the translation and rotation ambiguity by dolly-zoom effect and distortion scale.}
% \label{fig:camera}
\end{figure}



This procedure rearrangeed the image feature in a structured way. This structured information is more  making it less varing comparing to various feautre distrubution of $F_{img}$. 

In practice, we utilize DensePose\cite{Guler2018DensePose} for $M_{iuv}$ prediction. We rearrange the part $UV$ map given by DensePose into a whole feautre map according to different part's relation, as shown in fig. \ref{fig:camera}

We emperically think these arrangement could preserve more neighboring body-part relationships. While DecoMR\cite{decomr} proposed an continuous UV map that is whole-body unfold, the IUV map estimation methods based on this UV convention is less accurate. Experiments utilizing different GT IUV map also shows a close performance between these two UV configuration. 
\subsection{Wrapped Feature Completion}

The wrapped feature have a dense connection, but since the full $UV$ map is a map of the whole body-mesh, so the $\mathbf{F_{UV} } \in \mathbb{R}^{D \times H \times W}$ wrapped from a single image has at least 50 \% blank area, since at least 50 \% of the mesh surface is invisible. 
 The wrapped feature completion module aims at utilize the visible features to reason the occluded features. Then it will extract body-part wise feature through soft-attention. 

We first use convolution blocks to downsample the wrapped feature map, and fuse the neighboring features. This could fuse the features within a body part, and around the neighboring parts. We also want the module to consider a long range communication between different parts. To model this connection, we propose an attention method to further refer features from different body parts. Based on the downscale $UV$ feature map after convolution, we apply two convolution layer $W_A, W_V$ to the downsample feature map $F^{d}_{UV}$ to derive body part attention weight $\mathcal{A}$ and attention value$\mathcal{V}$. Then, we weighted sum the attention value through element-wise matric muliplication formualted as:
\begin{equation}
F_i^p=\sum_{h,w}\sigma(\mathcal{A_i}) \circ \mathcal{V}
\end{equation}
where $\circ$ denotes element-wise multiplication and $\sigma$ is softmax function.



\subsection{UV Based Feature Inpainting}


Using feature wrapping and feature completion techniques, we have obtained an accurate part-wise feature vector. Our goal is to ensure that these features are robust and invariant to occlusions, denoted as $F_i^p$. Previous methods have relied on data augmentation strategies, such as random cropping or synthetic occlusion, to achieve this goal. However, experiments conducted by Pang et al. \cite{pang2022benchmarking} indicate that such augmentation methods may not be as helpful as previously believed. Furthermore, we recognize that it is challenging for the network to learn completion without any intermediate supervision.

To address this issue, we propose a feature inpainting training method that provides part-wise supervision for occlusion augmentation. Specifically, we input both the occluded and original images to the network and wrap their features with occluded and original IUV maps. We then obtain two distinct sets of part-wise features from the UV completion module, denoted as $F^{po}$ and $F^{p}$. For the occluded feature $F^{po}$, our objective is to make its vector similar to the unoccluded feature vector $F^{p}$, thereby enabling the network to learn how to fill these feature vectors. We model this as a similarity loss formulated as:
\begin{equation}
    L_{sim}=\frac{1}{p} \sum_{i=0}^{p-1} \frac{F^{po}_i F^{p}_i}{|F^{po}_i||F^{p}_i|}
\end{equation}

In traning, we only retain the gradient of the occluded feature vector. With this training methods the model was able to learn more accurate human pose when parts are occluded, compared to simple occlusion augmentation.

\subsection{Loss functions}
We flatten the part feature $F_i^p$, and concatenate them with global feautre $F^g$, initial SMPL and camera parameters $(\boldsymbol{\theta}, \boldsymbol{\beta}, \boldsymbol{\pi})_{init}$. And regress the final parameters $(\boldsymbol{\theta}, \boldsymbol{\beta}, \boldsymbol{\pi})$ in a iterative regressison manner. We supervised our training with SMPL parameters loss $L_{SMPL}$, 3D keypoints loss $L_{3D}$,  2D keypoints $L_{2D}$ and similarity loss $L_{sim}$ that can be formulated as:
\begin{equation}
 \begin{aligned}
L =\lambda_{S M P L} L_{S M P L}+\lambda_{3 D} L_{3 D}+\lambda_{2 D} L_{2 D}
+\lambda_{sim} L_{sim}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
&L_{S M P L}=\|(\boldsymbol{\theta}, \boldsymbol{\beta})-(\boldsymbol{\hat\theta}, \boldsymbol{\hat\beta)}\|, \\
L_{3 D}=&\left\|J_{3 D}-\hat{J}_{3 D}\right\|, 
L_{2 D}=\left\|J_{2 D}-\hat{J}_{2 D}\right\|,
\end{aligned}
\end{equation}
where $J_{2 D}=s \Pi(R  W\mathcal{M}(\boldsymbol{\theta}, \boldsymbol{\beta}))+t. $
The ground truth SMPL parameters are obtained from Mosh data or pseudo-fitting depending on the datasets. We obtained $J_{2 D} \in \mathbb{R}^{J \times 2}$ with the following equation: $J_{2 D}=s \Pi(R  W\mathcal{M}(\boldsymbol{\theta}, \boldsymbol{\beta}))+t$


\subsection{Implementation Details}
We train DIMR for xxx steps with batch size 64, using Adam optimizer with a learning rate of 5e-5. The backbone we used are ResNet50 pretrained on COCO pose etimation, and HRNet pretrained on COCO pose estimation. We first train our model without parallel inpainting. Then we finetune them with sythetic occlusion.



==> sections/5-discussion.tex <==

\section{Discussion.}
Although our model achieves SOTA performance on occlusion datasets, its performance is heavily influenced by the predicted IUV map. An accurate IUV map can greatly increase the performance of our model. But this design couldn't improve the quality of IUV with training. In the future, a built-in dense map prediction module trained with the network might solve this problem. But we have to specially design the module to achieve occlusion robustness. 

==> sota-3dpw.tex <==
\begin{table}
    \centering
     \scalebox{0.7}{
        \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{\textbf{Methods}} &\multirow{2}{*}{Backbone}&
        \multirow{2}{*}{w. 3DPW} 
        & \multicolumn{3}{c}{Metrics}\\ \cmidrule{4-6}
        & &  & PA-MPJPE$\downarrow$ & MPJPE$\downarrow$ & PVE$\downarrow$  \\ 
        \midrule 

        HybrIK\cite{hybrik} &  ResNet-34 & $\times$ & 48.8  & 80.0  & 94.5  \\
        HybrIK\cite{hybrik} &  ResNet-34 &$\checkmark$ & 45.0  & 74.1  & 86.5  \\
        GraphCMR~\cite{graphcmr} & ResNet-50  & $\times$  &70.2  & - &    - \\
        HMR~\cite{hmr} & ResNet-50 & $\times$ &72.6  &  116.5 & -         \\
        SPIN~\cite{spin}  &  ResNet-50 &$\times$ & 59.2     & 96.9    &116.4\\
        PyMarf~\cite{pymaf}  & ResNet-50  & $\times$ & 58.9 & 92.8  & 110.1   \\
        SPEC~\cite{spec}  &  ResNet-50  & $\checkmark$ & 52.7  & 96.4  & -  \\
        PARE~\cite{pare}  &  ResNet-50 & $\times$ &  52.3 & 82.9  & 99.7\\


        FastMetro~\cite{fastmetro} &  ResNet-50  &$\checkmark$ & 48.3  & 77.9  & 90.6  \\
        CLIFF~\cite{cliff}  &  ResNet-50   &$\checkmark$ & 45.7  & 72.0  & 85.3   \\
        PARE~\cite{pare}  &  HRNet-w32 & $\checkmark$ & 46.5 &  74.5 &88.6 \\
        CLIFF~\cite{cliff}  &  HRNet-w48 & $\checkmark$ & 43.0 & 69.0 & 81.2        \\
        Graphormer~\cite{meshgraphormer}  &  HRNet-w64 &$\checkmark$& 45.6  & 74.7  & 87.7   \\
        FastMetro~\cite{fastmetro} &  HRNet-w64  &$\checkmark$ & 44.6  & 73.5  & 84.1    \\


        \midrule
        \Ours  & ResNet-50  & $\times$&    48.9      & 80.0 & 92.3\\
        \Ours   & HRNet-w48  & $\times$ & &        &\\
        \Ours   & HRNet-w48  & \checkmark & 46.8 & 77.6        & 94.7 \\
        \bottomrule
        \end{tabular} 
    }
    \vspace{-0.05in}
    \caption{Results of SOTA methods on 3DPW
    }
    \vspace{-2ex}
 %   \vspace{-1ex}
    \label{tab:pdhuman-mtp}
\end{table}

==> sota-distortion.tex <==
\begin{tabular}{lccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c}{PDHuman ($TH_{d}^{3.0}$)}& \multicolumn{5}{c}{SPEC-mtp ($TH_{d}^{1.8}$)}
&\multicolumn{5}{c}{HuMMan($TH_{d}^{1.8}$)}\\ \cmidrule{2-16}
&MPJPE$\downarrow$ & PA-MPJPE$\downarrow$  & PVE$\downarrow$ & mIoU$\uparrow$ &P-mIoU$\uparrow$& MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ & PVE$\downarrow$ & mIoU$\uparrow$ &P-mIoU$\uparrow$& MPJPE$\downarrow$ & PA-MPJPE$\downarrow$ & PVE$\downarrow$ &  mIoU$\uparrow$  & P-mIoU$\uparrow$ \\ \midrule 

\rule{0pt}{10pt} HMR~(R50)~\cite{hmr} & 91.5   & 62.5  & 106.7  & 48.9 & 21.7& 121.4  & 73.9  & 145.6  & 48.8  & 16.0 &  43.6 & 30.2   & 52.6 & 65.1   & 39.5 \\

\rule{0pt}{10pt} SPEC~(R50)~\cite{spec} &  94.9 & 65.8 &109.6 & 43.4   & 19.6  & 125.5  & 76.0  &144.6 &  49.9 & 18.8  & 44.0  & 31.4  & 54.2 & 51.4 & 25.6       \\

\rule{0pt}{10pt} CLIFF~(R50)~\cite{cliff} & 99.2  &66.2  &  115.2  &51.4  & 24.8  &  115.0 & 74.3    & 132.4 & 53.6  &23.7  &42.4   &28.6 &50.2  &68.8   & 44.7\\

% SPIN~(R50)~\cite{spin} &   &  &  &   &   &  &    & &   &  &   & &   &  \\



\rule{0pt}{10pt} PARE~(H48)~\cite{pare}  & 95.9  & 66.3  & 116.7 & 48.2    & 20.9   & 121.6 &74.2    & 143.6 & 55.8   & 23.2  & 53.2  & 32.6 & 65.5  & 66.5 & 38.3  \\

% CLIFF~(H48)~\cite{cliff} &   &  &  &    &   &  &   &  &   &  &   &   &   & \\
% PARE (H48) &   &  &    & &   &  &   & & \\

% PyMarf~\cite{pymaf}   &   &  &   &  &   &   &   &  &   &  &   &    &   &  \\
% HybrIK~\cite{hybrik}   &   &  &   &  &   &   &   &  &   &  &   &  &   &    \\
\midrule
\rule{0pt}{10pt} GraphCMR~(R50)   & 85.8  & 62.0  & 98.4  & 47.9    & 21.5  & 121.4  &  76.1   & 141.6  &  53.5 & 22.0 &  40.6 & 29.5  & 48.4  & 61.6 & 37.5   \\

\rule{0pt}{10pt} FastMetro(H48)~\cite{fastmetro}   & 87.7  & 61.7 & 100.1 & 50.9  & 23.8  & 125.7  & 75.2    & 140.5 & 53.7  & 19.8  & 38.8 & 26.3  & 45.5  & 68.3 & 45.2    \\

\midrule
\rule{0pt}{10pt} \Ours (R50)& 80.9   & 54.3 & 93.9  & 54.5  & 27.4 & 117.6   & 72.9 &     138.2 & 54.7 & 22.4  & 36.7 &24.3 & 45.9 & 70.4 & 45.5   \\
\rule{0pt}{10pt} \Ours (H48)  &   &  &  &  &   &  &  &   &  &  &   &   \\
\bottomrule
\end{tabular}


==> tables/sota-3dpw.tex <==
\begin{table}
    \centering
     \scalebox{0.7}{
        \begin{tabular}{lccccc}
        \toprule
        \multirow{2}{*}{\textbf{Methods}} &\multirow{2}{*}{Backbone}&
        \multirow{2}{*}{w. 3DPW} 
        & \multicolumn{3}{c}{Metrics}\\ \cmidrule{4-6}
        & &  & PA-MPJPE$\downarrow$ & MPJPE$\downarrow$ & PVE$\downarrow$  \\ 
        \midrule 

        HybrIK\cite{hybrik} &  ResNet-34 & $\times$ & 48.8  & 80.0  & 94.5  \\
        HybrIK\cite{hybrik} &  ResNet-34 & $\times$ & 48.8  & 80.0  & 94.5  \\
        HybrIK\cite{hybrik} &  ResNet-34 &$\checkmark$ & 45.0  & 74.1  & 86.5  \\
        GraphCMR~\cite{graphcmr} & ResNet-50  & $\times$  &70.2  & - &    - \\
        HMR~\cite{hmr} & ResNet-50 & $\times$ &72.6  &  116.5 & -         \\
        SPIN~\cite{spin}  &  ResNet-50 &$\times$ & 59.2     & 96.9    &116.4\\
        PyMarf~\cite{pymaf}  & ResNet-50  & $\times$ & 58.9 & 92.8  & 110.1   \\
        SPEC~\cite{spec}  &  ResNet-50  & $\checkmark$ & 52.7  & 96.4  & -  \\
        PARE~\cite{pare}  &  ResNet-50 & $\times$ &  52.3 & 82.9  & 99.7\\


        FastMetro~\cite{fastmetro} &  ResNet-50  &$\checkmark$ & 48.3  & 77.9  & 90.6  \\
        CLIFF~\cite{cliff}  &  ResNet-50   &$\checkmark$ & 45.7  & 72.0  & 85.3   \\
        PARE~\cite{pare}  &  HRNet-w32 & $\checkmark$ & 46.5 &  74.5 &88.6 \\
        CLIFF~\cite{cliff}  &  HRNet-w48 & $\checkmark$ & 43.0 & 69.0 & 81.2        \\
        Graphormer~\cite{meshgraphormer}  &  HRNet-w64 &$\checkmark$& 45.6  & 74.7  & 87.7   \\
        FastMetro~\cite{fastmetro} &  HRNet-w64  &$\checkmark$ & 44.6  & 73.5  & 84.1    \\


        \midrule
        \Ours  & ResNet-50  & $\times$&    48.9      & 80.0 & 92.3\\
        \Ours   & HRNet-w48  & $\times$ & &        &\\
        \Ours   & HRNet-w48  & \checkmark & 46.8 & 77.6        & 94.7 \\
        \bottomrule
        \end{tabular} 
    }
    \vspace{-0.05in}
    \caption{Results of SOTA methods on 3DPW
    }
    \vspace{-2ex}
 %   \vspace{-1ex}
    \label{tab:pdhuman-mtp}
\end{table}

==> tables/sota-h36m.tex <==
\begin{table}[]
\begin{tabular}{cc|ccc}
\toprule
\small
\multicolumn{2}{c|}{\multirow{2}{*}{Methods}}   & \multicolumn{3}{c}{H36M}   \\ 
                            \cline{3-5} 
         &                 & PA-MPJPE$\downarrow$ & MPJPE$\downarrow$ & PVE$\downarrow$  \\ 

\midrule

\multirow{6}{*}{\rotatebox{90}{General}}
                        & DecoMR~\cite{decomr}                  & 61.7     & -     & -     \\
                        & SPIN~\cite{spin}                    & 59.2     & 96.9  & 116.4  \\
                        & PyMAF~\cite{pifu}                   & 58.9     & 92.8  & 110.1 \\
                        & HMR-EFT~\cite{eft}                 & 52.2     & 85.1  & 98.7\\
                        & METRO~\cite{metro}                   & 47.9     & 77.1  & 88.2 \\

\hline

\multirow{4}{*}{\rotatebox{90}{Occludsion}}  
                                & OCHMR~\cite{ochmr}                   & 58.3     & 89.7  & 107.1\\
                                & Pose2UV~\cite{pose2uv}                 & 57.1     & -     & -  \\
                                & ROMP~\cite{romp}                    & 53.3     & 85.5  & 103.1 \\
                                & PARE~\cite{pare}                    & 50.9     & 82    & 97.9 \\
                                
\hline
& DIMR (Ours)                    & 52.9     & 87    & 106.6 \\
& DIMR (GT IUV)                 & 47.8    & 73.0 & 99.5 \\
\bottomrule

\end{tabular}
\vspace{0.05in}
\caption{\textbf{Quantitative comparison results} with state-of-the-art methods on 3DPW. We compare the performance of our method with competing for general methods and occlusion-aware methods. } 
\end{table}
